An overview of the efficiency and censorship-resistance guarantees of widely-used consensus protocols

Censorship resistance with short-term inclusion guarantees is an important feature of decentralized systems, missing from many state-of-the-art and even deployed consensus protocols. In leader-based protocols the leader arbitrarily selects the transactions to be included in the new block, and so does a block builder in protocols such as Bitcoin and Ethereum. In a different line of work, since the redundancy of consensus for implementing distributed payments was formally proven, consensusless protocols have been described in theory and deployed in the real world. This has resulted in blockchains and payment systems that are more efficient, and at the same time avoid the centralized role of a leader or block builder. In this report we review existing consensus and consensusless protocols with regard to their censorship-resistance, efficiency, and other properties. Moreover, we present an approach for new constructions with these properties in mind, building on existing leader-based protocols.

==> macros.tex <==
\newcommand{\Ledger}{\mathbf{L}}
\newcommand{\LState}{\mathsf{L}}
\newcommand{\negl}{\textsf{negl}(\kappa)}
\newcommand{\view}{\textsc{view}}
\newcommand{\fullview}{\textsc{view}^{t,n}_{\Pi,\mathcal{A},\mathcal{Z}}}
\newcommand{\validityattack}{\textsc{persistence}\textsc{-}\textsc{game}}
\newcommand{\livenessattack}{\textsc{liveness}\textsc{-}\textsc{game}}
\newcommand{\true}{\ensuremath{\mathsf{true}}\xspace}
\newcommand{\false}{\ensuremath{\mathsf{false}}\xspace}
\newcommand{\approxn}{\widetilde{n}}
\DeclareMathOperator{\diff}{\textsf{diff}\,}
\newcommand{\dexpand}[1]{#1_{\pm\Delta}}
\newcommand{\cert}{\ensuremath{\pi}\xspace}

\newcommand{\concat}{\,\|\,}
\newcommand{\eg}{\emph{e.g., }}

\hyphenation{log-a-rith-mic}
\hyphenation{unique-ly}
\hyphenation{ex-tractabil-i-ty}

\algnewcommand\algorithmicon{\textbf{upon}}
\algblockdefx[ON]{On}{EndOn}[1]
{\algorithmicon\ #1\ \algorithmicdo}
{\algorithmicend\ \algorithmicon}

\algnewcommand\waitcommand{\textbf{wait until }}
\def\Wait#1{\State\waitcommand #1}

\def\chain{\mathcal{C}}
\DeclareMathOperator{\Ex}{\mathbb{E}}

\newcommand{\getsrandomly}{\overset{\$}{\gets}}


\newcommand{\condtext}[1]{{\ifhide\else #1 \fi}}
\newcommand{\oa}[1]{{\color{blue}{ \condtext{OA: #1}}}}
\newcommand{\bd}[1]{{\color{olive}{ \condtext{BD: #1}}}}
\newcommand{\wip}[1]{{\hue{WIP: #1}}}


\newcommand{\op}[1]{\textsl{#1}}
\newcommand{\opwrite}[1]{\op{write(#1)}\xspace}
\newcommand{\opwriteret}[1]{\op{write\_return(#1)}\xspace}
\newcommand{\opwritedeps}[1]{\op{store(#1)}\xspace}
% \newcommand{\opread}[1]{\op{read(#1)}\xspace}
\newcommand{\opreadall}[1]{\op{read\_perfect(#1)}\xspace}
\newcommand{\opreadallret}[1]{\op{read\_perfect\_return(#1)}\xspace}
\newcommand{\opreaddirty}[1]{\op{read\_all(#1)}\xspace}
\newcommand{\opreaddirtyret}[1]{\op{read\_all\_return(#1)}\xspace}
\newcommand{\opgetdeps}[1]{\op{get\_deps(#1)}\xspace}
\newcommand{\opidentify}[1]{\op{identify(#1)}\xspace}
\newcommand{\opbcast}[1]{\op{broadcast(#1)}\xspace}
\newcommand{\opdel}[1]{\op{deliver(#1)}\xspace}
\newcommand{\opsign}[1]{\op{Sign(#1)}\xspace}
\newcommand{\opmin}[1]{\op{min(#1)}\xspace}
\newcommand{\opmax}[1]{\op{max(#1)}\xspace}
\newcommand{\opmed}[1]{\op{med(#1)}\xspace}
\newcommand{\opvalid}[1]{\op{valid(#1)}\xspace}
\newcommand{\opdisperse}[1]{\op{disperse(#1)}\xspace}
\newcommand{\opretrieve}[1]{\op{retrieve(#1)}\xspace}


\newcommand{\operand}[1]{\textsf{#1}}
\newcommand{\tx}{\operand{tx}\xspace}
\newcommand{\deptx}{\operand{deptx}\xspace}
\newcommand{\deptxid}{\operand{txid}\xspace}
\newcommand{\txid}{\operand{txid}\xspace}
\newcommand{\round}{\operand{r}\xspace}
\newcommand{\rexp}{\ensuremath{\round_\text{exp}}\xspace}
\newcommand{\rrec}{\ensuremath{\round_\text{rec}}\xspace}
\newcommand{\rmin}{\ensuremath{\round_\text{min}}\xspace}
\newcommand{\rmax}{\ensuremath{\round_\text{max}}\xspace}
\newcommand{\rinterval}{\ensuremath{[\rmin, \rmax]}\xspace}
\newcommand{\rreported}{\ensuremath{\round_\text{rep}}\xspace}
\newcommand{\rperf}{\ensuremath{\round_\text{perf}}\xspace}
\newcommand{\rloc}{\ensuremath{\round_\text{loc}}\xspace}
\newcommand{\txmiss}{\ensuremath{\txset_\text{miss}}\xspace}
\newcommand{\txfinal}{\ensuremath{\txset_\text{final}}\xspace}
\newcommand{\inclist}{\ensuremath{L}\xspace}
\newcommand{\gossipT}{\ensuremath{t_\text{prop}}\xspace}
\newcommand{\gossipC}{\ensuremath{c_\text{gos}}\xspace}
\newcommand{\txsize}{\ensuremath{s}\xspace}
\newcommand{\dadisp}{\ensuremath{t_\text{disp}}\xspace}
\newcommand{\daretr}{\ensuremath{t_\text{ret}}\xspace}
\newcommand{\dacom}{\ensuremath{c_\text{da}}\xspace}

\newcommand{\user}{\operand{user}\xspace}
\newcommand{\timestamp}{\operand{ts}\xspace}
\newcommand{\Cert}{\ensuremath{\Pi}\xspace}
\newcommand{\txset}{\operand{T}\xspace}
\newcommand{\final}{\operand{f}\xspace}
\newcommand{\parack}{\ensuremath{u}\xspace}
\newcommand{\parwrite}{\ensuremath{v}\xspace}
\newcommand{\parwiggle}{\ensuremath{W}\xspace}
\newcommand{\POD}{\ensuremath{D}\xspace}
\newcommand{\limbo}{\ensuremath{L}\xspace}

\newcommand{\returns}{\ensuremath{\rightarrow}\xspace}
\newcommand{\dotparagraph}[1]{\paragraph*{#1.}}
\newcommand{\hue}[1]{\textcolor{brown}{#1}}
\newcommand{\recorded}{recorded\xspace}
\newcommand{\finalized}{finalized\xspace}
\newcommand{\zo}{\ensuremath{\{ 0, 1\}\xspace}}

% for pseudocode
\newcommand{\return}{\State{\textbf{return}}\xspace}
\newcommand{\st}{\textbf{such that}\xspace}
\newcommand{\andl}{\textbf{and}\xspace}
\newcommand{\msgwrite}{\text{WRITE}\xspace}
\newcommand{\msgread}{\text{READ}\xspace}
\newcommand{\msgprecommit}{\text{PRECOMMIT}\xspace}

